S-RAN: Semantic-Aware Radio Access Networks

Semantic communication (SemCom) has been a transformative paradigm, emphasizing the precise exchange of meaningful information over traditional bit-level transmissions. However, existing SemCom research, primarily centered on simplified scenarios like single-pair transmissions with direct wireless links, faces significant challenges when applied to real-world radio access networks (RANs). This article introduces a Semantic-aware Radio Access Network (S-RAN), offering a holistic systematic view of SemCom beyond single-pair transmissions. We begin by outlining the S-RAN architecture, introducing new physical components and logical functions along with key design challenges. We then present transceiver design for end-to-end transmission to overcome conventional SemCom transceiver limitations, including static channel conditions, oversimplified background knowledge models, and hardware constraints. Later, we delve into the discussion on radio resource management for multiple users, covering semantic channel modeling, performance metrics, resource management algorithms, and a case study, to elaborate distinctions from resource management for legacy RANs. Finally, we highlight open research challenges and potential solutions. The objective of this article is to serve as a basis for advancing SemCom research into practical wireless systems.

==> knowledge.tex <==
Knowledge management is significant in S-RAN since semantic encoder and decoder both rely on accumulative knowledge for semantics extraction and recovery. 

\subsection{Knowledge Construction and Embedding} 

For an individual user, three fundamental processes for knowledge construction in S-RAN should be considered: knowledge extraction (KE), knowledge representation learning (KRL), and knowledge graph completion (KGC). The initial step involves extracting valuable entities and relations from raw data. This is accomplished through algorithms for named entity recognition (NER) and relation extraction, culminating in the formation of triples—comprising head entities, relations, and tail entities. Following extraction, the next step is to map these triples into vectors, translating intricate human-understandable knowledge into a structured format digestible by machines. However, the persistent issue of incomplete triples during KB construction should not be overlooked. Therefore, KGC algorithms aim to predict and fill in the missing information in these incomplete triples \cite{vu2019capsule}.

Once we complete knowledge construction for each user, we next should focus on the embedding of the knowledge to increase the reasoning ability and generalizability of S-RAN. In the transceiver design, the special tokens (e.g., names, locations and events) can be first aligned to the entities in knowledge graph (entity-relation-entity). Then, the indexes of entities associated to their triples are embedded into the tokens for training encoders/decoders. 

\subsection{Knowledge Sharing and Update}

KBs are strategically distributed across device layer, access layer, and server layer within S-RAN. Dynamic sharing and updating mechanisms are indispensable to maintain knowledge freshness and consistency. 
\begin{itemize}
    \item Sharing knowledge between transmitter and receiver can improve coding and transmission efficiency since the understanding ability at both side could be at the same level. Moreover, sharing among different nodes enables collective learning and cooperative knowledge creation, often facilitated by methods like federated learning.
    \item To maintain the accuracy and relevance of the Knowledge Base (KB) community, regular audits and updates are conducted to identify and remove outdated or incorrect data. The incorporation of up-to-date knowledge serves two key purposes: 1) it enables efficient utilization of limited storage on devices, and 2) it enhances semantic accuracy during transmission using fewer bits. However, the integration of updated knowledge also presents new challenges in transceiver design, particularly as learning models employed in transceivers are typically pre-trained based on previous knowledge.  
\end{itemize}

(we can have a case study as well based on that V2X paper, depending on word budget.)
